Making Scalable Meta Learning Practical

Despite its flexibility to learn diverse inductive biases in machine learning programs, meta learning (i.e., learning to learn) has long been recognized to suffer from poor scalability due to its tremendous compute/memory costs, training instability, and a lack of efficient distributed training support. In this work, we focus on making scalable meta learning practical by introducing SAMA, which combines advances in both implicit differentiation algorithms and systems. Specifically, SAMA is designed to flexibly support a broad range of adaptive optimizers in the base level of meta learning programs, while reducing computational burden by avoiding explicit computation of second-order gradient information, and exploiting efficient distributed training techniques implemented for first-order gradients. Evaluated on multiple large-scale meta learning benchmarks, SAMA showcases up to 1.7/4.8x increase in throughput and 2.0/3.8x decrease in memory consumption respectively on single-/multi-GPU setups compared to other baseline meta learning algorithms. Furthermore, we show that SAMA-based data optimization leads to consistent improvements in text classification accuracy with BERT and RoBERTa large language models, and achieves state-of-the-art results in both small- and large-scale data pruning on image classification tasks, demonstrating the practical applicability of scalable meta learning across language and vision domains.

==> experiments.tex <==
\section{Experiments}
\label{sec:experiments}
In this section, we scale up three popular meta learning applications with SAMA: 1. data optimization, 2. data pruning, and 3. model-agnostic meta learning. In doing so, we attempt to (a) evaluate the scalability of SAMA compared to existing approaches, (b) study the effectiveness of each component in SAMA, and (c) investigate the potential of scalable meta learning in various applications. Since the main theme of this work is making scalable meta learning \textit{practical}, we intentionally avoid using high-end GPUs (\textit{e}.\textit{g}.,\ NVIDIA A100), but rather distribute compute/memory across multiple lower-end GPUs (\textit{e}.\textit{g}., NVIDIA 2080Ti) with our communication-efficient strategy when needed.
We provide all experiment details including hyperparameters and compute resources in Appendix B.

\subsection{Large-Scale Data Optimization}
One of the major assumptions underlying most machine learning programs is that training data provide strong inductive biases that represent test data from the target task. Nonetheless, such assumptions are often invalidated especially in real-world machine learning scenarios for a variety of reasons, such as distribution shift or label noise, and the model learned on wrong data performs poorly when it is deployed. Meta learning can be a powerful tool to mitigate this issue, by optimizing training data given a small amount of high-quality test data. In this work, we in particular explore two scenarios, namely (i) noisy label learning and (ii) auxiliary learning, both of which suffer from distribution mismatch between training and test data distributions. 

\subsubsection{Noisy Label Learning: Weak Supervision Finetuning of Large Language Model}
Weak supervision~\cite{ratner2016data} proposes to achieve a significant reduction in the data labeling cost by letting users quickly generate labels for a large amount of data by exploiting multiple weak labeling functions, such as hand-designed rules and other neural networks. While increasing the \textit{quantity} of labeled data with weak supervision has led to noticeable improvements in multiple applications, a poor \textit{quality} of generated labels results in a degradation in test accuracy, leaving the room for further improvement. Here, we attempt to alleviate this data quality issue in weak supervision by utilizing meta learning to automatically optimize noisy training data guided by a small amount of clean data in the meta level. In detail, we use data reweighting~\cite{shu2019meta} and label correction~\cite{zheng2021meta} as our data optimization operations, of which the bilevel optimization formulation is as follows:
\begin{align*}
    &\lambda^* = (\lambda_{r}^*, \lambda_c^*)=\underset{\lambda_{r}, \lambda_c}{\mathrm{argmin}}\;\mathcal{L}(D_{clean};\theta^*(\lambda_{r}, \lambda_c))\\
    \text{s.t. }\theta^*(\lambda_r, \lambda_c)=\;&\underset{\theta}{\mathrm{argmin}}\;\frac{1}{|D_{train}|}\sum_{(x,y)\in D_{noisy}}w(\mathcal{L};\lambda_r)\cdot \mathcal{L}(f(x_i;\theta), c(x_i, y_i; \lambda_c))
\end{align*}
where $w(\cdot;\lambda_r)$ and $c(\cdot;\lambda_c)$ are meta learners, respectively, for data reweighting and label correction.
To evaluate the scaling efficiency of SAMA, we perform text classification with a BERT-base model with 110M parameters on multiple weak supervision datasets from the WRENCH benchmark~\cite{zhang2021wrench}. Furthermore, to study the effectiveness of our algorithmic adaptation trick (Sec 3.2), we conduct experiments with a variant of SAMA (\textit{i}.\textit{e},.\ SAMA-NA), which doesn't include an algorithmic adaptation, and present every experiment result in Table~\ref{tab:wrench}.
\begin{table}[!ht]
\footnotesize
\centering
\begin{tabular}{lccccccc}
\toprule
          & Algorithm & TREC  & SemEval & IMDB  & ChemProt & AGNews & YouTube \\\midrule
Baseline  & -       & 67.93\tiny{ (2.55)} & 79.28\tiny{ (1.78)}   & xx.xx\tiny{ (y.yy)} & 57.35\tiny{ (1.43)}    & 85.79\tiny{ (0.49)}  & 92.27\tiny{ (0.92)}   \\
\midrule
+R      & SAMA-NA   & 74.33\tiny{ (2.34)} & 87.11\tiny{ (1.11)}   & xx.xx\tiny{ (y.yy)} & 60.88\tiny{ (0.60)}    & 86.83\tiny{ (0.19)}  & 94.40\tiny{ (0.40)}   \\
+R \& C & SAMA-NA   & 79.00\tiny{ (2.62)} & 87.67\tiny{ (1.36)}   & xx.xx\tiny{ (y.yy)} & 64.05\tiny{ (0.52)}    & 87.05\tiny{ (0.39)}  & 95.33\tiny{ (0.23)}   \\
\midrule
+R      & SAMA    & 85.73\tiny{ (0.81)} & \textbf{89.67}\tiny{ (0.67)}   & xx.xx\tiny{ (y.yy)} & 76.89\tiny{ (1.39)}    & 89.05\tiny{ (0.34)}  & 95.73\tiny{ (2.01)}   \\
+R \& C & SAMA    & \textbf{87.93}\tiny{ (1.17)} & 88.83\tiny{ (2.32)}   & xx.xx\tiny{ (y.yy)} & \textbf{77.78}\tiny{ (0.59)}    & \textbf{89.79}\tiny{ (0.27)}  & \textbf{96.13}\tiny{ (0.83)}  \\
\bottomrule
\end{tabular}
\vskip 5pt
\caption{WRENCH results. R and C in the first column stand for data reweighting and label correction operations. SAMA-NA does not use algorithmic adaptation (Sec 3.2) for Adam optimizer. A small number in the parentheses is standard deviation for each experiment.}
\label{tab:wrench}
\end{table}
\vskip -15pt

In this experiment we are able to make two observations. First, we notice that meta-learning-based data reweighting and label correction lead to consistent improvements in noisy text classification accuracy of the \textit{large} Transformer model across all benchmarks. Second, given the superior performance of SAMA compared to SAMA-NA, we empirically verify the importance of algorithmic adaption (Sec 3.2) when an adaptive optimizer is used to train this Transformer base learner.
% the large Transformer-based base learner.

\begin{wraptable}{R}{5.5cm}
{\scriptsize
\begin{tabular}{cccc}
\toprule
        & GPUs & Memory & Throughput \\\midrule
Neumann & 1    & 26008  & 82.90      \\[0.3ex]
CG      & 1    & 28418  & 82.05      \\[0.3ex]
SAMA-NA & 1    & 13710  & 144.14     \\[0.3ex]
SAMA    & 1    & 14332  & 142.01     \\[0.3ex]
SAMA    & 2    &        &            \\[0.3ex]
SAMA    & 4    &        &            \\\bottomrule
\end{tabular}
\vskip -3pt
\caption{Memory and throughput analysis on AGNews with 4 V100 GPUs.}
\label{tab:system}
}
\end{wraptable}
Additionally, we compare compute/memory efficiency of SAMA to that of two other implicit-differentiation-based meta learning algorithms, namely Neumann Series~\cite{lorraine2020optimizing} and conjugate gradient~\cite{rajeswaran2019meta}. For fair comparison, we evaluate GPU memory usage (GiB) and throughput (samples/sec) on the AGNews dataset from Wrench with a fixed \textit{global} batch size of 48, and summarize the result in Table~\ref{tab:system}. Three observations that can be made here are that (1) SAMA is generally more compute/memory efficient than the baselines, (2) the cost of algorithmic adaptation for adaptive optimizers is marginal as expected, and (3) the efficiency gap further widens as we distribute compute/memory across multiple GPUs with our efficient DDP communication strategy. Since we were only able to conduct experiments with up to 4 V100 GPUs due to the limited compute resources, exploring extremely large-scale GBML with larger GPU servers remains as a promising future research direction.

\subsubsection{Auxiliary Learning: Continued Pretraining of Large Language Models}
DAPT/TAPT~\cite{gururangan2020don} empirically demonstrate that additionally pretraining (\textit{i}.\textit{e}.,\ continued pretraining) the generic language model on the domain or task specific data could further improve the downstream performance on diverse benchmarks. However, since pretraining and downstream tasks are essentially from different distributions, there still is a potential of negative transfer~\cite{wang2019characterizing} from a part of pretraining data, which could lead to a suboptimal downstream performance. Here, we attempt to minimize such negative transfer by reweighting samples from the continued pretraining task with meta learning. To this end, we adopt the auxiliary learning technique from TARTAN~\cite{dery2021should} and simplify the two-stage pretraining-finetuning pipeline into the one-stage multitask learning pipeline with the reweighting scheme applied to the pretraining loss, of which bilevel optimization formulation is as follows:
{\small
\begin{align*}
    \lambda^*&=\underset{\lambda}{\mathrm{argmin}}\;\mathcal{L}_{ft}(D_{ft};\theta^*(\lambda))\\
    \text{s.t. }\theta^*(\lambda)&=\underset{\theta}{\mathrm{argmin}}\;\mathcal{L}_{ft}(D_{ft};\theta)+\frac{1}{|D_{pt}|}\sum_{x\in D_{pt}}w(x;\lambda)\cdot \mathcal{L}_{pt}(x;\theta)
\end{align*}}where $\mathcal{L}_{ft}$/$\mathcal{L}_{ft}$ is finetuning/pretraining loss functions, $D_{ft}$/$D_{pt}$ are finetuning/pretraining datasets,  $w(\cdot;\lambda)$ is the data reweighting network. Unlike the original TARTAN work where they learned one global importance weight for the auxiliary task, we learn importance weights for all \textit{tokens} in the auxiliary pretraining task with neural networks to gain more fine-grained control over information transfer. Accordingly, the dimension of meta parameters (\textit{i}.\textit{e}.,\ inductive biases) is much higher in our experiments. Given this setup, we run our experiments with the large RoBERTa-base model on 3 benchmarks from \cite{dery2021should,gururangan2020don}, and provide the experiment results in Table~\ref{tab:tapt}.
\begin{table}[!ht]
\centering
{\small
\begin{tabular}{lcccccc}
\toprule
                   & Baseline & TAPT~\cite{gururangan2020don} & TARTAN-MT~\cite{dery2021should} & TARTAN-Meta~\cite{dery2021should} & Multi-Task & SAMA\\\midrule
ChemProt & 82.1 \tiny{(1.0)}       & 82.6 \tiny{(0.4)}     & 84.3 \tiny{(0.6)}            & 84.5 \tiny{(0.5)}       & xx.x \tiny{(1.0)}      & xx.x \tiny{(1.0)}         \\[0.5ex]
ACL-ARC  & 63.0 \tiny{(5.8)}       & 67.4 \tiny{(1.8)}      & 70.5 \tiny{(4.4)}            & 70.1 \tiny{(4.7)}        & xx.x \tiny{(1.0)}      & xx.x \tiny{(1.0)}       \\[0.5ex]
SCIERC   & 77.3 \tiny{(1.9)}       & 79.3 \tiny{(1.5)}      & 80.8 \tiny{(0.7)}            & 81.5 \tiny{(0.8)}       & xx.x \tiny{(1.0)}      & xx.x \tiny{(1.0)}         \\\bottomrule
\end{tabular}
}
\vskip 5pt
\caption{Experiment results for auxiliary learning with the continued pretraining task. Following \cite{gururangan2020don}, we report test micro-F1 for ChemProt and macro-F1 for the other datasets. A small number in the parentheses is standard deviation for each experiment.}
\label{tab:tapt}
\end{table}
\vskip -13pt

\sang{@Sanket please write some discussion. @Sanket please write some discussion.@Sanket please write some discussion.@Sanket please write some discussion.@Sanket please write some discussion.@Sanket please write some discussion.@Sanket please write some discussion.@Sanket please write some discussion.@Sanket please write some discussion.@Sanket please write some discussion.@Sanket please write some discussion.@Sanket please write some discussion.@Sanket please write some discussion.}

\subsection{Scale-Agnostic Efficient Data Pruning}
Data pruning~\cite{paul2021deep,sorscher2022beyond,toneva2018empirical,wang2023dynams} has recently received the limelight in the machine learning community as a means to both improve training efficiency and reduce (semantic) redundancy in training data. In particular, Sorscher et al.~\cite{sorscher2022beyond} showed both theoretically and experimentally that  neural scaling laws can be beaten by data pruning. Nevertheless, they point out that the optimal data pruning metric varies across different dataset scales and further research in scalable data pruning metric is needed. Here, we propose to forgo hand-designed data pruning metrics, and rather automatically \textit{meta-learn} the importance weight of each training data following Meta-Weight-Net (MWN)~\cite{shu2019meta} with three major modifications. First, we replace their iterative differentiation meta gradient algorithm with SAMA. In doing so, we are able to achieve improved memory/compute efficiencies, especially with larger unroll steps. Second, we further speed up meta learning by enabling distributed training with our communication optimization technique. Third, we use the uncertainty of the prediction in addition to the loss value as an input to MWN to better estimate importance weight of each training data. A bilevel optimization formulation of our method is as follows:
{\small
\begin{align*}
    \lambda^*&=\underset{\lambda}{\mathrm{argmin}}\;\mathcal{L}(D_{train};\theta^*(\lambda))\\
    \text{s.t. }\theta^*(\lambda)&=\underset{\theta}{\mathrm{argmin}}\;\frac{1}{|D_{train}|}\sum_{(x,y)\in D_{train}}w(\mathcal{L},\,\mathcal{U};\lambda)\cdot \mathcal{L}(x, y;\theta)
\end{align*}}where $w(\cdot;\lambda)$ is MWN that takes the loss value $\mathcal{L}$ and the uncertainty $\mathcal{U}$ of the training sample $(x,y)$ as an input and outputs the importance weight. Under this setup, we run meta learning with SAMA for 30 / 50 epochs respectively for ImageNet-1k / CIFAR-10, and obtain the pruning metrics by averaging the importance weights of last 5 epochs. We compare our method to several popular static/dynamic data pruning baselines, and present the results in Figure~\ref{fig:pruning}.

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.49\linewidth]{figures/imagenet-1.pdf}
    \includegraphics[width=0.49\linewidth]{figures/cifar.pdf}
    \vskip 3pt
    {\scriptsize
    \begin{tabular}{lcccccc}
    \toprule
                 & EL2N$_1$~\cite{paul2021deep} & EL2N$_{10}$~\cite{paul2021deep} & GradNd$_{10}$~\cite{paul2021deep} & DynaMS~\cite{wang2023dynams} & MWN~\cite{shu2019meta} & SAMA (ours)\\\midrule
    Relative Search Time  & 0.16      & 1.65       & 1.65     & 0.16     & xx & xx  \\\bottomrule
    \end{tabular}}
    \caption{\textbf{Top Left:} ImageNet-1k data pruning results with ResNet-50. Reported numbers are relative accuracy compared to full training accuracy (\textit{i}.\textit{e}.,\ pruned\_acc/full\_acc). Accuracy for other baseline methods is obtained from DynaMS~\cite{wang2023dynams}. \textbf{Top Right:} CIFAR-10 data pruning results with ResNet-18. Accuracy for other baseline methods is obtained from Deepcore~\cite{guo2022deepcore}. \textbf{Bottom:} Relative time spent in finding data to prune compared to full ImageNet-1k training time.}
    \label{fig:pruning}
\end{figure}

% As we expected above, GBML-based data pruning (\textit{i}.\textit{e}.,\ SAMA)
As expected, GBML-based data pruning with SAMA
not only outperforms heuristics-based data pruning, but also works well across different dataset scales. Surprisingly, we observe that GBML-based data pruning even leads to improvements in test accuracy at the pruning ratio of 0.1 and 0.2 on ImageNet-1k. The potential implication is that ImageNet-1k may have noisy labels or semantic redundancy, and that GBML is able to automatically figure and filter out these samples. Further in-depth investigation on filtered data remains as an interesting research direction. Considering that compute/memory inefficiency has traditionally been the major bottleneck in GBML applications, we also compare the relative search time for data pruning. Unlike iterative-differentiation-based MWN which suffers from considerably long search time, our efficient SAMA demonstrates comparable or even shorter search time than heuristics-based methods.



\subsection{Model-Agnostic Meta Learning: Scale vs Algorithm}
Since the inception of MAML~\cite{finn2017model}, a myriad of algorithms have been proposed to improve few-shot image classification while assuming the fixed network architecture. In contrast, we here shift our focus from the algorithm to the scale, and propose to study the following question: ``Leveraging the compute/memory efficiency of SAMA, can we improve the few-shot generalization capability by scaling up the network size?''. Since SAMA is a variant of implicit differentiation, we closely follow the experiment setup in iMAML~\cite{rajeswaran2019meta}, where proximity to the initialization weights is explicitly enforced by $L_2$-regularization. The major difference is that iMAML uses a conjugate-gradient-based method, which requires second-order gradient information to compute meta gradients, while we adopt SAMA to achieve improved scaling to larger networks with its superior memory/compute efficiency.  We conduct experiments on the Omniglot dataset with the basic 4-layer CNN architecture, while varying the width (hidden size) of the networks to study the effect of the model size on the few-shot classification accuracy. The experiment results are provided in Table~\ref{tab:maml}.

\begin{table}[!ht]
\centering
{\small
\begin{tabular}{lccccccccc}
\toprule
      &      & \multicolumn{4}{c}{5-way}                               & \multicolumn{4}{c}{20-way}                              \\\cmidrule(r){3-6}\cmidrule(r){7-10}
Algorithm  & Width & \multicolumn{2}{c}{1-shot} & \multicolumn{2}{c}{5-shot} & \multicolumn{2}{c}{1-shot} & \multicolumn{2}{c}{5-shot} \\\cmidrule(r){3-4}\cmidrule(r){5-6}\cmidrule(r){7-8}\cmidrule(r){9-10}
      &       & Acc         & Memory       & Acc         & Memory       & Acc         & Memory       & Acc         & Memory       \\\midrule
MAML\cite{finn2017model}  & 64    & 98.7       & yyyy         & 99.9       & yyyy         & 95.8       & yyyy         & 98.9       & yyyy         \\[0.3ex]
iMAML\cite{rajeswaran2019meta} & 64    & 99.16       & yyyy         & 99.67       & yyyy         & 94.46       & yyyy         & 98.69       & yyyy         \\[0.3ex]
SAMA  & 64    & xx.xx       & yyyy         & xx.xx       & yyyy         & xx.xx       & yyyy         & xx.xx       & yyyy         \\[0.3ex]
SAMA  & 256   & xx.xx       & yyyy         & xx.xx       & yyyy         & xx.xx       & yyyy         & xx.xx       & yyyy         \\[0.3ex]
SAMA  & 1024  & xx.xx       & yyyy         & xx.xx       & yyyy         & xx.xx       & yyyy         & xx.xx       & yyyy         \\\bottomrule
\end{tabular}
}\vskip 5pt
\caption{Omniglot few-shot image classification accuracy and GPU memory usage with varying algorithms and model sizes.}
\label{tab:maml}
\end{table}

Since SAMA doesn't require any computation involving the Hessian, it demonstrates better memory efficiency compared to other algorithms, allowing us to scale up the width (\textit{i}.\textit{e}.\ size) all the way up to 1024. Interestingly, we observe that the increased model size also leads to consistent improvements in few-shot classification accuracy. The important question following this observation is ``Can we apply scaling laws~\cite{kaplan2020scaling} from other tasks (\textit{e}.\textit{g}.,\ language modeling) to general meta learning beyond few-shot image classification?'' Since meta learning involves two optimization problems (meta and base) unlike traditional machine learning problems, it is as of now unclear how to define the general concept of ``scale'' in terms of both model and dataset sizes. We expect that further research in this direction would be critical in systematically studying scalable meta learning.
